The Visibility Center of a Simple Polygon

We introduce the \emph{visibility center} of a set of points inside a polygon -- a point $c_V$ such that the maximum geodesic distance from $c_V$ to see any point in the set is minimized. For a simple polygon of $n$ vertices and a set of $m$ points inside it, we give an $O((n+m) \log {(n+m)})$ time algorithm to find the visibility center. We find the visibility center of \emph{all} points in a simple polygon in $O(n \log n)$ time. Our algorithm reduces the visibility center problem to the problem of finding the geodesic center of a set of half-polygons inside a polygon, which is of independent interest. We give an $O((n+k) \log (n+k))$ time algorithm for this problem, where $k$ is the number of half-polygons.

==> 150_Basics.tex <==
Our region of interest is a simple polygon $P$ with $n$ vertices whose boundary $\partial P$ is directed clockwise.
A \textit{chord} $K = ab$ of a simple polygon is a straight line segment joining two points $a,b \in \partial P$ such that the segment $ab$ does not intersect $\partial P$ at any point except $a$ and $b$.
Every chord $ab$ gives rise to two half-polygons---one containing the clockwise boundary between $a$ and $b$ and the other containing the clockwise boundary between $b$ and $a$.
We will denote by the ordered pair $(a,b)$ the half-polygon defined by chord $ab$ that contains the clockwise boundary between $a$ and $b$.




\medskip
\noindent
\textbf{Geodesic Distance.} The \emph{geodesic distance} $d(x,y)$ (or simply, \textit{distance}) between two points in a simple polygon $P$ is the length of a shortest path joining them that lies within the interior of $P$.
The \textit{shortest path} between two points $x,y$ that lies within the interior of $P$ is unique and is denoted $\pi(x,y)$~\cite{lee1984euclidean}.
We will also use the term \textit{geodesic} to refer to shortest paths.















\medskip
\noindent
\textbf{Geodesic Centers.}
Given a set of points $S \subseteq P$ and a point $x \in P$, the distance $d(x,S)$ is defined as: $\min\limits_{s \in S} d(x,s)$.
It is possible that the geodesic distance between $x$ and a point set $S$ is realized at multiple points of $S$.
For the case of segments, there is a unique shortest path $\pi(x,s)$ from a point $x$ to a segment $s$. The point at which the distance to $s$ is realized is the \textit{terminal} $t(x,s)$.

Given the above definition of distance, we can proceed to define a geodesic center $c(\mathcal{S})$ of a set $\mathcal{S}$ of objects $S_1,S_2,\dots$.
A geodesic center of set $\mathcal{S}$ is any point inside the polygon $P$ that minimizes the distance to the furthest object of $\mathcal{S}$.
The distance to the furthest object of the set $\mathcal{S}$ from a point $x \in P$ is the \emph{geodesic radius} $r(x,\mathcal{S})$.
Thus, the geodesic center is a any element of $\argmin \{ r(x,\mathcal{S}) : x \in P  \}$.

In this paper, we will discuss how to determine a geodesic center of a set $\mathcal{H}$ of half-polygons of $P$.
Our techniques extend those of Pollack et al.~\cite{pollack_sharir} and are general enough to yield the geodesic centers of any set of convex polygonal objects inside a simple polygon.
If we restrict ourselves to a set $Q \subseteq P$, then a point in $Q$ that minimizes the maximum distance to any object in the set $\mathcal{S}$, is called the \textit{relative center of} $\mathcal{S}$ \textit{with respect to} $Q$.











 \medskip
 \noindent
\textbf{Convexity. }A subset $S$ of $P$ is \textit{geodesically convex} in $P$ if, for any two points $x,y \in S$, the geodesic $\pi(x,y) \subseteq P$.
The next lemma, about the convexity of the distance to a segment justifies the use of an oracle based method of determining the g


\begin{figure}[H]
\centering
\includegraphics[width=0.7\textwidth]{figures/convexity_proof-cropped.pdf}
\caption{Proving that $d(x,s)$ is a convex function of $d(a,x)$. $a'$ is the point where $\pi(a,b)$ diverges from $\pi(a,s)$ ($b'$ is defined similarly).
The angle $\theta (t)$ increases as we move from $a$ to $b$.
Convexity of the function in $\pi(a,c)$ and $\pi(d,b)$ was proven by Pollack et al.~\cite{pollack_sharir}.
For segments, their reasoning carries forward as shown in the proof of Lemma~\ref{lemma:geodesic_convexity_dist_to_element}.
}
\label{fig:proof_1}
\end{figure}

\begin{lem}\label{lemma:geodesic_convexity_dist_to_element}
As we move a point $x$ along $\pi(a,b)$ from $a$ to $b$, the geodesic distance $d(x,s)$ to a segment $s$ is a convex function of $d(a,x)$.
\end{lem}
\begin{proof}
The points on $\pi(a,b)$ from which the path to segment $s$ is a straight line segment are a continuous subpath $\pi(c,d)$ on $\pi(a,b)$ (See Figure~\ref{fig:proof_1}).
For $\pi(a,c)$ and $\pi(d,b)$, the proof of Pollack et al.~\cite{pollack_sharir} already shows that $d(x,s)$ for points in $ [a,c) \cup (d,b]$ is a convex function of $d(a,x)$.
For points between $c$ and $d$, we provide a proof sketch that proves the convexity for points on $\pi(c,d)$.


Let $t = d(a,x)$ and $\psi (t) = d(x,s)$. We need to show that $\psi(t)$ is a convex function between $c$ and $d$.
Let $u(x,y)$ denote the vector in the direction of the first segment on $\pi(x,y)$.
Let $\theta (t)$ denote the angle between $u(x,b)$ and $u(x,s)$.
Similarly, $\overline{\theta} (t)$ denotes the angle between $u(x,s)$ and $u(x,a)$.
Both these angles vary continuously as $x$ moves from $a$ to $b$ and take on values between $0$ and $\pi$ (except possibly at $c$, $d$).


We will prove that at every point a left derivative ($\psi_{-} '(t)$) and a right derivative ($\psi_{+} '(t)$) both exist with $\psi_{-} '(t) \leq \psi_{+} '(t)$.
Then we will prove that the right derivative is increasing between $c$ and $d$.
Both these facts together imply that $\psi(t)$ is convex.

It is easy to check that as we move away from $c$ the distance between $s$ and a segment of $\pi(c,d)$ varies linearly with a slope $- \cos{\theta(t)}$.
Thus the right hand derivative $\psi_{+} '(t) = - \cos{\theta(t)}$.
Similarly, the left derivative is $\psi_{-} '(t) = - \cos{\overline{\theta}(t)}$.
These values match the derivative values when the path to $s$ have turns.
As  $ \overline{\theta}(t) \geq \pi - \theta(t) $, we have $\psi_{-} '(t) \leq \psi_{+} '(t)$.

We can also show using the angle sum properties of a simple polygon that the value $\theta(t)$ must be increasing (not always strictly increasing, as in the case when we consider geodesic distance to a point as opposed to a segment).
This proves that the right derivative $\psi_{+} '(t) = - \cos{\theta(t)}$ must be increasing, proving the lemma.
\end{proof}





















\subsection{Concepts Related to Visibility}\label{section:concepts_visibility}

Two points $x,y \in P$ are \emph{visible} to each other if the line segment $xy$ lies in the interior of the polygon $P$.
For any point $u \in P$,  the set of all the points in $P$ visible from $u$ define the \emph{visibility polygon} $P_V(u)$.
Any edge of $P_V(u)$ that is not part of the boundary $\partial P$ is a \emph{window} that is determined by a reflex vertex $r$ of $P$ visible from $u$ and is formed by extending the ray  $\overrightarrow{ur}$ from the \emph{base} $r$ until it hits  $\partial P$ at the \emph{tip}.
We use $w(u,r)$ to denote this window.
The subpolygon cut off by $w(u,r)$ that contains $u$ and $P_V(u)$ is called the \emph{half-polygon} associated with $u$ and $r$, and is denoted $H(u,r)$.
The complement of the half-polygon is the \emph{pocket} $\overline{H}(u,r)$ associated with $u$ and $r$.


For points $x,u \in P$, the \emph{distance to visibility}, denoted $d_V(x,u)$, is the geodesic distance from $x$ to $P_V(u)$.
If $x \in P_V(u)$, then $d_V(x,u)$ = 0.
Otherwise, $x$ lies in some pocket $\overline{H}(u,r)$ and $d_V(x,u)$ is the geodesic distance from $x$ to the half-polygon $H(u,r)$.
A point of $H(u,r)$ that is geodesically nearest to $x$ in the latter case must lie on the window $w(u,r)$.
By Lemma~\ref{lemma:geodesic_convexity_dist_to_element}, this point is unique and we have a unique \emph{shortest path to visibility}, denoted $\pi_V(x,u)$.
The \emph{visibility radius} of a point $x$ with respect to a point set $U$ is: $r_V(x,U) = \max \{d_V(x,u) : u \in U\}$.
A \emph{visibility center} of $U$ is any element of $\argmin \{r_V(x,U): x \in P\}$.









\medskip
\noindent
\textbf{Kernel of a Point Set in $P$. }The kernel $\mathcal{K}(U)$ of a point set $U \subseteq P$ is the set of points from which all points of $U$ are visible.
If the kernel $\mathcal{K}(U)$ of a point set $U$ is non-empty, any point in the kernel is a visibility center.
The kernel of $m$ points inside a simple polygon with $n$ vertices can be determined in $O(n + m \log (m+n))$ time~\cite{ke1989computing}.
In the special case where we wish to compute the visibility center of a simple polygon, we can compute the kernel of an $n$ vertex simple polygon in linear time using an algorithm of Lee and Preparata~\cite{lee1979optimal}.
If the kernel is non-empty, any point in it qualifies as the visibility center.


In other words, we assume in what follows:
\begin{assumption}\label{assumption:empty_kernel}
The input to our algorithm has an empty kernel.
\end{assumption}



\medskip
\noindent
\textbf{Observations on the Visibility Center of a Simple Polygon. }
The following lemma helps to `discretize' the problem of finding the visibility center of a simple polygon:
\begin{lem}
Let $P$ be a polygon with an empty kernel.
The visibility radius $r_V(x)$ from any $x \in P$ is realized at the neighbor of reflex vertex of $P$.
\end{lem}
\begin{proof}
Let $u$ be a point in $P$ such that $d_V(x,u) = r_V(x)$.
If $u$ is the neighbor of a reflex vertex, we are done; so, let us suppose $u$ is not a reflex neighbor.

Consider the pocket $\overline{H}(u,r)$ defined by $u$ and the reflex vertex $r$ that contains $x$.
Exactly one neighbor (say, $r^-$) of $r$ is contained in the half-polygon $H(u,r)$ defined by $u$ and $r$.
Since the half-polygon $H(r^-,r) \subseteq H(u,r)$, we have $r_V(x) \geq d_V(x,r^-) \geq d_V(x,u) = r_V(x)$.
Thus, the visibility radius from $x$ is realized at $r^-$, a neighbor of the reflex vertex $r$.
This proves the lemma.
\end{proof}

\begin{coro}\label{corollary:vis_center_of_poly_is_vis_center_reflex_nbrs}
The visibility center of a simple polygon coincides with the visibility center of the set of all the vertices of $P$ that are neighbors of reflex vertices.
\end{coro}

As a result, the problem of finding a visibility center for a simple polygon reduces to finding the visibility center of the point set $U$ that consists of the neighbors of its reflex vertices.






==> 510_Functions_to_capture_distance_to_furthest_wedge.tex <==









In this section we give a linear time algorithm to find a linear number of simple functions defined on the chord $K=ab$ whose upper envelope is the geodesic radius function $r(x,{\cal H})$ for $x \in K$. 
Specifically, we use the shortest path trees 
$\bar T_a$ and $\bar T_b$ constructed in the previous section
to build a set of $O(n +k)$ pairs $f,I$ where: 
\begin{itemize}
\item 
$I$ is a subinterval of $K$ and $f$ is a function defined on domain $I$, 
\item each function has the form $f(x) = d_2(x,s) + \kappa$ where $\kappa$ is a constant,
$d_2$ is Euclidean distance, and  
$s$ is a point or a line,
\item for any point $x \in K$ the maximum of $f(x)$ over intervals $I$ containing $x$ is equal to $r(x,{\cal H})$.
\end{itemize}

For intuition, see Figure~\ref{fig:intervals-functions}, which shows several intervals and their associated functions. 
Note that we deal separately with the two pieces of the polygon on each side of $K$.
There is an obvious set of $O(nk)$ pairs $f,I$ with the above properties, one for each $H \in {\cal H}$ and $v \in P$, but we want a set of linear size.
















The crucial property is 
that there are a limited number of farthest half-polygons associated with each vertex, and we can restrict our attention (mostly) to longest paths in the trees $\bar T_a$ and $\bar T_b$.
In particular, consider a  point $x \in  K$, a half-polygon $H$, and the shortest path  $\pi(x,H)$.  Suppose  $\pi(x,H)$ has at least two edges, say 
$\pi(x,H) = x,u, v,\ldots, t$, where $t$ is the terminal point on $H$.
If $\pi(x,H)$ turns left 
at $u$, then the  part of the  path  from $u$ to $t$ is  part of the tree $\bar T_a$, and symmetrically for right turns and $\bar T_b$.
See Figure~\ref{fig:path-in-tree}.
Furthermore, if $H$ is a farthest half-polygon from $x$,  %
then we  can show 
\newcomment{(in the full version)}
that %
the  part of the  path from $v$ to $t$ is the  longest path in $\bar T_a$ descending from $v$ to any half-polygon.
Note that using longest paths from $u$ rather than  $v$ is not correct---see  Figure~\ref{fig:path-in-tree}. 


\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
  \centering
\includegraphics[width=\linewidth]{figures/intervals-functions.pdf}
\caption{}
\label{fig:intervals-functions}
\end{subfigure}
\hfill
\begin{subfigure}{0.4\textwidth}
  \centering
\includegraphics[width=\linewidth]{figures/path-in-tree-2.pdf}
\caption{}
\label{fig:path-in-tree}
\end{subfigure}
\caption{
(a) An illustration of functions and intervals. For $x$ in interval $I_1$, $d(x,H_1) = d_2(x,u) + \kappa_1$. For $x$ in $I_2$, $d(x,H_1) = d_2(x,v) + \kappa_2$.  For $x$ in $I_3$, $d(x,H_2) = d_2(x,H_2)$.
(b) From point $x$ the farthest half-polygon is $H_1$ via the path $x,u,v,t_1$.  This matches the longest path in $\bar T_a$
descending from $v$ (which goes to $H_1$) but does not match the longest path descending from $u$ (which goes to $H_2$).  
}
\end{figure}

For any node $u$ in $\bar T_a$ %
let $\ell_a(u)$
be the maximum length of a path in $\bar T_a$ descending from $u$ to a  node %
representing a terminal point on some half-polygon.
Define $\ell_b(u)$ similarly.
We can compute these functions in linear time in leaf-to-root order. 
In the situation described above, where $H$ is a farthest half-polygon from $x$ and the path $\pi(x,H) = x, u, v, \ldots, t$ turns left at $u$, we have $d(x,H) = 
|xu| + |uv| + \ell_a(v)$, which is a simple function of the desired form.


The algorithm will output these functions for all pairs $u,v$ where the following conditions hold: $u$ is a vertex visible from a point on the chord $ab$ (equivalently, 
$u$ has different parents in $\bar T_a$ and $\bar T_b$);
$v$ is a child of $u$ in one of the trees; and $x$ lies in an appropriate interval on $ab$ such that $u,v$ can be the start of a geodesic path from $x$.
We deal separately with 
shortest paths that go from a point $x \in ab$ to a half-polygon without going through any vertices. 
Observe that the number of such functions is $O(n+k)$.

We defer further details of the algorithm to 
\revised{Appendix~\ref{appendix:functions}.}
Besides enhancing the method of Pollack et al.~\cite{pollack_sharir} to deal with half-polygons, 
our aim is to give a clearer and easier-to-verify presentation.





==> 800_Points_In_a_Polygon.tex <==
\section{Visibility Center for Points in a Simple Polygon}

\subsection{Introduction}
In this work, we initiate a study of the \textit{visibility center}---a point in a given polygon domain starting from which we do not have to move too much to \textit{see} any of a given set $M$ of target points.
Our model of visibility is the same as the one used in art gallery problems; two points in the domain see each other if the straight line segment joining them does not properly intersect the domain boundary or a pre-defined set of obstacles.
By a \textit{path} joining a two points $x,y$ in the polygonal domain, we mean a path connecting $x$ and $y$ that does not intersect the boundary or any obstacles.
The geodesic distance between two points is the length of the shortest path joining them.
The geodesic distance between a point $x$ and some set $S$ is the length of a shortest path joining $x$ to some point in $S$.


Various facility location problems have been studied in computational geometry.
These include geodesic centers (that minimize the maximum geodesic distance to reach any point in a polygonal domain) and link centers (that minimize the maximum bends in a polygonal path to any point in a polygonal domain).
However, literature on paths to visibility and facility location problems related to these is surprisingly sparse.

In the visibility center problem, we wish to find a point starting from which the maximum distance to visibility over all points in a target set $M$ is minimized.
This has potential applications for facility location problems involving line of sight communications or defense / surveillance type applications where a target only needs to be seen (rather than reached) for it to be serviced.
We may also think of this as an art gallery problem with a single mobile guard---we want to ensure that the maximum distance the guard has to move to respond to an emergency is minimized.



We look at the simplest case of this problem when the domain is a simple polygon with points from the set $M$ in its interior.
The only obstacle is the boundary of the simple polygon itself.
The visibility center $c_V(M)$ of a set of points in a polygon $P$ is shown in Figure~\ref{fig:figure_with_visibility_center}.

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figures/show_cv-cropped.pdf}
\caption{Given a set $M$ of points inside $P$, $c_V(M)$ is their visibility center.}
\label{fig:figure_with_visibility_center}
\end{figure}


\subsection{Definitions}
The radius to visibility $r_V(x,M)$ from a starting point $x \in P$ for the set of points $M$ is defined as: $r_V(x,M):= \max\limits_{u \in M} \{d_V(x,u)\}$.
In this case, we define a visibility center $c_V(M)$ to be any point in the set $\underset{x \in P}{\argmin}\{r_V(x,M)\}$.
For any given point $x \in P$, the distance to visibility $d_V(x,u)$ equals the geodesic distance $d(x,P_V(u))$ from $x$ to the visibility polygon $P_V(u)$.
Thus the visibility center $c_V(M)$ is a point that minimizes the maximum geodesic distance to any visibility polygon in the set $\mathcal{P}_V(M) = \{P_V(u) \mid u \in M\}$.



\begin{figure}
\centering
\includegraphics[width=0.65\textwidth]{figures/visibility_concepts-cropped.pdf}
\caption{The visibility polygon $P_V(u)$ for the point $u$ is shown.
It naturally partitions $P$ into hidden subpolygons (unshaded polygons).
A hidden subpolygon $H(u,r)$ is defined by $u$ and a reflex vertex $r$.
It is separated from $P_V(u)$ by an aperture $a(u,r)$.
For any $x \in H(u,r)$, distance to visibility $d_V(x,u)$ equals the geodesic distance to the aperture $d(x,a(u,r))$.}
\label{fig:visibility_concepts}
\end{figure}

\subsection{The Furthest Aperture Recognition Problem}
The construction of a visibility polygon for a point $x$ takes $O(n)$ time~\cite{el1981linear}.
If we begin by constructing each visibility polygon for points in the set $M$, the algorithm will take $\Omega(mn)$ time.
We will avoid this expensive construction and use a more efficient approach.

Recall from Section~\ref{section:concepts_visibility} that the visibility polygon $P_V(u)$ for any point $u$ partitions $P$ into hidden subpolygons and $P_V(u)$ (See Figure~\ref{fig:visibility_concepts}).
For any point in $P_V(u)$, the distance to visibility is zero.
Any point $x$ outside of $P_V(u)$ lies in a hidden subpolygon $H(u,r)$ defined by the aperture $a(u,r)$.
The aperture is constructed by extending the ray $\overrightarrow{u,r}$ until it hits $\partial P$ for the first time.
The aperture $a(u,r)$ has two endpoints---the reflex vertex $r$ that we call the fulcrum of the aperture, and the result of the ray shooting that we call the image $im(u,r)$ of the aperture.
The aperture $a(u,r)$ is said to be active for $x \in H(u,r)$ with respect to the point $u$ and is unique for any point $x \notin P_V(u)$.
All points in $H(u,r)$ are said to lie on the \textit{hidden side} of aperture $a(u,r)$.
All points in $P \setminus H(u,r)$ are said to lie on the \textit{visible side} of $a(u,r)$.

We have the following:
\begin{center}
$d_V(x,u) = d(x,P_V(u)) = d(x,a(u,r))$    
\end{center}

Suppose we had prior knowledge about the apertures defined by points in set $M$ that were active with respect to a visibility center $c_V(M)$.
In such a situation, we could ignore the visibility polygons of points in set $M$ and work with the less complicated apertures that are simply chords of the polygon.
We now want to solve the following \emph{furthest aperture recognition problem}:

\noindent
\textbf{Given a set $M$ of $m$ points within a simple polygon $P$ with $n$ vertices, find a small ($O(n)$ sized) set of apertures that is a superset of the furthest apertures from $c_V(M)$.}

We begin with a series of observations:
\begin{obs}\label{observation:point_in_hidden_subpolygon__is_captured}
Consider the hidden subpolygon $H(u,r)$ that is formed by joining a point $u \in P$ to a reflex vertex $r$ visible from it.
The last link on the shortest path $\pi(x,u)$ joining a point $x \in H(u,r)$ to $u$ must contain the segment $[r,u]$.
\end{obs}

\begin{proof}
The subpolygon $H(u,r)$ is separated from $P \setminus H(u,r)$ by the aperture $a(u,r)$.
So, the path $\pi(x,u)$ must cross the aperture at some point $y \in a(u,r)$.
Since the shortest path within $P$ from $y$ to $u$ is a straight line segment, the last link must be the segment $[y,u]$, which must contain $[r,u]$.
\end{proof}


\begin{obs}\label{observation:one_aperture_endpoint_in_hidden_subpolygon}
Suppose we $a_1 = a(u_1,r_1)$ and $a_2=a(u_2,r_2)$ are two furthest apertures from $c_V(M)$ with $r_1 \neq r_2$.
At least one endpoint of $a_1$ (resp. $a_2$) must lie in $H(u_2,r_2)$ (resp. $H(u_1,r_1)$).
In other words, neither $H(u_1,r_1)$ nor $H(u_2,r_2)$ contains the other.
\end{obs}

\begin{proof}
Consider the paths $\pi(c_V(M),a_1)$ and $\pi(c_V(M),a_2)$.
If both endpoints of $a_1$ belong to $P \setminus H(u_2,r_2)$, then the path to $a_1$ will cross $a_2$ and hence must necessarily be longer.
This contradicts the fact that both path lengths are equal.
\end{proof}


\begin{obs}\label{observation:furthest_apertures_point_on_visible_side}
Suppose we $a_1 = a(u_1,r_1)$ and $a_2=a(u_2,r_2)$ are two furthest apertures from $c_V(M)$ with $r_1 \neq r_2$.
If $u_2 \notin H(u_1,r_1)$, then $r_2 \notin H(u_1,r_1)$.
\end{obs}
\begin{proof}
Suppose $u_2 \notin H(u_1,r_1)$ but $r_2 \in H(u_1,r_1)$.
Then the aperture $a(u_2,r_2)$ has a hidden subpolygon $H(u_2,r_2)$ that is completely contained within $H(u_1,r_1)$.
This means that the distance $d(c_V(M), a(u_2,r_2)) < d(c_V(M), a(u_1,r_1))$, contradicting the assumption that both apertures are furthest and hence equidistant from the visibility center.
\end{proof}


\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/two_points_same_fulcrum-cropped.pdf}
\caption{Figure depicting the situation where Observation~\ref{observation:apertures_with_same_reflex_vertex} holds.
Points $u_1$ and $u_2$ have the same reflex vertex that defines the aperture for point $x \in P$.
The direction of the hidden subpolygons is indicated.
In this case, the hidden subpolygon $H(u_2,r)$ contains $H(u_1,r)$.
Any path from $x$ to view $u_2$ must cross the aperture $a(u_1,r)$.}
\label{fig:two_points_same_fulcrum}
\end{figure}
\begin{obs}\label{observation:apertures_with_same_reflex_vertex}
If two apertures $a(u_1,r)$ and $a(u_2,r)$ have a common reflex vertex $r$ with respect to any point $x \in P$, either $H(u_1,r) \subseteq H(u_2,r) $ or $H(u_2,r) \subseteq H(u_1,r)$.
\end{obs}
\begin{proof}
Let the neighbor of the reflex vertex $r$ that lies in the hidden subpolygons be $n$ (See Figure~\ref{fig:two_points_same_fulcrum}).
The aperture that makes a greater angle with $\overrightarrow{r,n}$ has a subpolygon that contains the other. 
\end{proof}


\begin{claim}\label{claim:no_intersection_of_aperture_equals_catching_reflex}
Consider two furthest apertures $a_1 = a(u_1,r_1)$ and $a_2 = a(u_2,r_2)$  from $c_V(M)$.
If $a_1$ and $a_2$ do not intersect, the shortest path $\pi(u_1,u_2)$ joining $u_1$ and $u_2$ must contain the reflex vertices $r_1$ and $r_2$.
\end{claim}

\begin{proof}
We know that the apertures $a_1$ and $a_2$ do not have any common points.
Furthermore, the visibility center $c_V(M)$ under consideration lies in the intersection of hidden subpolygons $H_1 = H(u_1,r_1)$ and $H_2 = H(u_2,r_2)$.

Due to Observation~\ref{observation:one_aperture_endpoint_in_hidden_subpolygon}, we know that neither $H(u_1, r_1)$ nor $H(u_2, r_2)$ can be completely contained within the other.

Since $a_1$ and $a_2$ do not intersect, the only other possibility is $a_1 \in H_2$ and $a_2 \in H_1$.
This should mean that $u_1 \in H_2$ and $u_2 \in H_1$.
Observation~\ref{observation:point_in_hidden_subpolygon__is_captured} then tells us that $[r_1,u_1]$ lies on the path $\pi(u_2, u_1)$ and, symmetrically, $[r_2, u_2]$ lies on $\pi(u_1, u_2)$.
This proves our claim.
\end{proof}



\begin{claim}\label{claim:one_furthest_point_in_hidden}
Suppose that the visibility center $c_V(M)$ has at least three furthest apertures.
Let us denote these apertures by $a_1 = a(u_1,r_1)$, $a_2 = a(u_2,r_2)$ and $a_3=a(u_3,r_3)$.
At least one of the $u_i, i = 1,2,3$ lies in the hidden subpolygon $H(u_j,r_j), i\neq j, j = 1,2,3$.
\end{claim}


\begin{proof}
Without loss of generality, let us begin by assuming that $u_1 \notin H(u_2,r_2)$ and $u_2 \notin H(u_1,r_1)$.
This implies that the reflex vertex $r_2 \notin H(u_1,r_1)$ and $r_1 \notin H(u_2,r_2)$.
Therefore, by Observation~\ref{observation:one_aperture_endpoint_in_hidden_subpolygon}, the apertures $a_1$ and $a_2$ intersect each other.
A schematic showing the relative placement of the apertures is shown in Figure~\ref{fig:intersecting_apertures}.

Note that the visibility center $c_V(M)$ must lie in the intersection of the hidden subpolygons for each aperture.
Additionally, we suppose in the lemma that $u_3$ lies in the `non-hidden' side of both $u_1$ and $u_2$.
All possible locations for the aperture for $u_3$ result in either $u_1$ and $u_2$ being in the hidden subpolygon (let us call it $H_3$) defined by $u_3$ (see Figure~\ref{fig:intersecting_apertures}).
Thus, both $u_1$ and $u_2$ cannot lie in $P \setminus H_3$. At least one of them lies in $H_3$, proving the claim.

\begin{figure}
\centering
\includegraphics[width=0.65\textwidth]{figures/one_u_i_in_hidden_subpolygon-cropped.pdf}
\caption{Given that the apertures $a_1$ and $a_2$ intersect and contain $u_3$ on their `non-hidden' side, this figure shows the possibilities (green dashed lines) for the aperture defined by $a_3$.
For both configurations, we obtain a contradiction since at least one of $u_1, u_2$ must lie in its hidden subpolygon.}
\label{fig:intersecting_apertures}
\end{figure}
\end{proof}


\subsection{Algorithm for the Furthest Aperture Recognition Problem}
The following algorithm recognizes set $\mathcal{A}$ of $O(n)$ apertures of $P$ that is a superset of the furthest apertures from a visibility center $c_V(M)$:

\begin{algorithm}[H]\label{algorithm:aperture_recognition}
\DontPrintSemicolon
  
  \KwInput{Set of points $M$ inside a simple polygon $P$}
  \KwOutput{Set of Apertures $\mathcal{A}$ that is a superset of apertures $\mathcal{A}_{f}$ furthest from $c_V(M)$}
  \tcc{Relative Convex Hull: Phase 1}
  
  Construct the Relative Convex Hull $RCH(M)$ of $M$ with respect to $P$.
  
  For neighbors $m$ of reflex vertices $r$ of $RCH(M)$ that belong to the set $M$, shoot rays in the direction $\overrightarrow{mr}$ to find the first intersection point $i$ with $\partial P$.
  
  Define a new set $M' = M \cup I$ consisting of all the points in $M$ with the set $I$ that consists of the results of the ray shooting queries.
  
  
    
    \tcc{Relative Convex Hull: Phase 2}
    Construct the Relative Convex Hull $RCH(M')$ of $M'$ with respect to $P$.
    
    For neighbors $m \in M$ of reflex vertices $r'$ of $RCH(M')$, shoot rays in the direction
    $\overrightarrow{mr'}$ to find the first intersection point $i'$ with $\partial P$. Add the aperture $a(m,r') = r'i'$ to the set $\mathcal{A}$ of apertures.
    
    Return set $\mathcal{A}$.

\caption{Algorithm for the Furthest Aperture Recognition Problem}
\end{algorithm}

\begin{lem}
Algorithm~\ref{algorithm:aperture_recognition} correctly solves the furthest aperture recognition problem.
\end{lem}
\begin{proof}
Let the set of furthest apertures from a visibility center $c_V(M)$ be called $\mathcal{A}_{f}$.
Due to Observation~\ref{observation:apertures_with_same_reflex_vertex}, we restrict our attention to apertures that have different reflex vertices with respect to $c_V(M)$.
It is clear that the size of $\mathcal{A}_f$ is greater than one, since if there was just a single furthest aperture, we could move in its direction and strictly decrease the radius of visibility by a small amount.
This would contradict the assumption that $c_V(M)$ was the visibility center.

\textbf{Case 1 - At least three furthest apertures.} First, we consider the case when $|\mathcal{A}_f| \geq 3$.
Let $a(u_1,r_1)$, $a(u_2,r_2)$ and $a(u_3,r_3)$ represent three of the furthest apertures from the (unknown) visibility center $c_V(M)$.
We need to prove that Algorithm~\ref{algorithm:aperture_recognition} recognizes all of these apertures.
Suppose for contradiction that one of these apertures is not recognized by our algorithm, say $a(u_1,r_1)$.
Now, if $u_2$ lies in the hidden subpolygon $H(u_1,r_1)$, then Phase 1 of the relative convex hull must contain the vertex $r_1$ due to Observation~\ref{observation:point_in_hidden_subpolygon__is_captured}.
Thus if aperture $a(u_1,r_1)$ has not been recognized, $u_2 \notin H(u_1,r_1)$.
By Observation~\ref{observation:furthest_apertures_point_on_visible_side}, this means $r_2 \notin H(u_1,r_1)$.
This implies that the image $i(u_2,r_2)$ must lie in $H(u_1,r_1)$.

Now, if the reflex vertex $r_2$ was part of the relative convex hull in Phase 1 of the algorithm, $r_1$ would be a part of the relative convex hull in Phase 2 since the image $i(u_2,r_2)$ determined by ray shooting after Phase 1 lies in the hidden subpolygon $H(u_1,r_1)$.
Thus $r_2$ cannot be a vertex of the relative convex hull in Phase 1 of our algorithm.

This implies that $u_1 \notin H(u_2,r_2)$, $u_3 \notin H(u_1,r_1)$, and $u_3 \notin H(u_2,r_2)$ by Observation~\ref{observation:point_in_hidden_subpolygon__is_captured}.

Now we use Claim~\ref{claim:one_furthest_point_in_hidden} to conclude that either $u_1 \in H(u_3,r_3)$ or $u_3 \in H(u_3,r_3)$.
In any case, the relative convex hull of Phase 1 contains $r_3$.
However, this implies (Observation~\ref{observation:one_aperture_endpoint_in_hidden_subpolygon}) that when we shoot the ray $\overrightarrow{u_3,r_3}$ the image $im(u_3,r_3)$ is a part of both  $H(u_1,r_1)$ and $H(u_2,r_2)$.
However, this means that the relative convex hull from Phase 2 should contain fulcrum $r_1$, contradicting our assumption.
In other words, Algorithm~\ref{algorithm:aperture_recognition} recognizes the furthest apertures from $c_V(M)$ in this case.

\textbf{Case 2 - Two furthest apertures.} In this case, the furthest apertures cannot intersect. This means that both furthest apertures (let us call them $a(u_1,r_1)$ and $a(u_2,r_2)$) must lie in each other's hidden subpolygons.
This means that Phase 1 of our algorithm will detect the corresponding fulcrums and the furthest apertures are recognized by Algorithm~\ref{algorithm:aperture_recognition}.
This proves the lemma.
\end{proof}


